A Generalized LinDistFlow Model for Power Flow Analysis

This paper proposes a new linear power flow model for distribution system with accurate voltage magnitude estimates. The new model can be seen as a generalization of LinDistFlow model to multiphase distribution system with generic network topology (radial or meshed) around arbitrary linearization point. We have shown that the approximation quality of the proposed model strictly dominates that of the fixed-point linearization (FPL) method, a popular linear power flow model for distribution system analysis, when both are linearized around zero injection point. Numerical examples using standard IEEE test feeders are provided to illustrate the effectiveness of the proposed model as well as the improvement in accuracy over existing methods when linearized around non-zero injection points.

==> v0_BasedonCircuit.tex <==
% in the preamble:

\usepackage[standard]{ntheorem}

% later in the document:

\begin{Definition}[Tautology]\label{def:tautology}
A \emph{tautology} is a proposition that is always true for any value of its variables.
\end{Definition}

\begin{Definition}[Contradiction]\label{def:contradiction}
A \emph{contradiction} is a proposition that is always false for any value of its variables.
\end{Definition}

\begin{Theorem}
If proposition $P$ is a tautology then $\sim P$ is a contradiction, and conversely.
\begin{Proof}
If $P$ is a tautology, then all elements of its truth table are true (by Definition~\ref{def:tautology}), so all elements of the truth table for $\sim P$ are false, therefore $\sim P$ is a contradiction (by Definition~\ref{def:contradiction}).
\end{Proof}
\end{Theorem}

\begin{Example}\label{ex:rain}
``It is raining or it is not raining'' is a tautology, but ``it is not raining and it is raining'' is a contradiction.
\end{Example}

\begin{Remark}
Example~\ref{ex:rain} used De Morgan's Law $\sim (p \vee q) \equiv \sim p \wedge \sim q$.
\end{Remark}
